Deterministic Low-Diameter Decompositions for Weighted Graphs and Distributed and Parallel Applications

This paper presents new deterministic and distributed low-diameter decomposition algorithms for weighted graphs. In particular, we show that if one can efficiently compute approximate distances in a parallel or a distributed setting, one can also efficiently compute low-diameter decompositions. This consequently implies solutions to many fundamental distance based problems using a polylogarithmic number of approximate distance computations. Our low-diameter decomposition generalizes and extends the line of work starting from [Rozho\v{n}, Ghaffari STOC 2020] to weighted graphs in a very model-independent manner. Moreover, our clustering results have additional useful properties, including strong-diameter guarantees, separation properties, restricting cluster centers to specified terminals, and more. Applications include: -- The first near-linear work and polylogarithmic depth randomized and deterministic parallel algorithm for low-stretch spanning trees (LSST) with polylogarithmic stretch. Previously, the best parallel LSST algorithm required $m \cdot n^{o(1)}$ work and $n^{o(1)}$ depth and was inherently randomized. No deterministic LSST algorithm with truly sub-quadratic work and sub-linear depth was known. -- The first near-linear work and polylogarithmic depth deterministic algorithm for computing an $\ell_1$-embedding into polylogarithmic dimensional space with polylogarithmic distortion. The best prior deterministic algorithms for $\ell_1$-embeddings either require large polynomial work or are inherently sequential. Even when we apply our techniques to the classical problem of computing a ball-carving with strong-diameter $O(\log^2 n)$ in an unweighted graph, our new clustering algorithm still leads to an improvement in round complexity from $O(\log^{10} n)$ rounds [Chang, Ghaffari PODC 21] to $O(\log^{4} n)$.

==> 600-simple_applications.tex <==

\section{Simple and Standard Applications of our Results}

First, we state our main theorem. Then, we show how one can get some standard clusterings as its corollaries. 


As a corollary, we get the following variant of the theorem for cutting edges. 

\begin{theorem}[clustering for cutting edges]
\label{thm:steroids_edges}
\todo{fill}
Rewrite above for the case when we care about cutting edges. 
\end{theorem}
\begin{proof}
Put a new vertex in the middle of each edge $e$, with radius equal to $\ell(e)/2$. Hope for the best. 
\end{proof}


\paragraph{Standard Clusterings}


\begin{corollary}[Padded Well-Separated strong-radius Clustering]
\label{cor:separated_padded_clustering}
Let $G$ be a weighted graph and $\mu$ a weight function on its nodes and $D$ a parameter. 
Then there is an algorithm constructing a $D$-padded, $D$-separated clustering with strong-radius $\tO(D/\delta)$ such that the total weight of the set of miserable nodes $M$ is $\mu(M) \le \delta\mu(V(G))$. 
The algorithm needs access to a $(1+\eps)$-approximate tree-like distance oracle $\fO$ up to distance $\tO(D)$. It needs $\tO(1)$ aggregations along outputs of $\fO$ and $\tO(1)$ global aggregations. 
\end{corollary}
\begin{proof}
We use the last part of \cref{thm:steroids}. 
We set $D_\Tref{thm:steroids} = \tO(D)$ and $D'_\Tref{thm:steroids} = D$. 
We also use $S_\Tref{thm:steroids} = V(G)$,  $R_\Tref{thm:steroids} = 0$, and $\delta_\Tref{thm:steroids} = \delta$. 
\end{proof}


\begin{corollary}[Padded Well-Separated Neighborhood Covers]
Let $G$ be a weighted graph and $D$ a parameter. 
Then there is an algorithm constructing a sparse neighborhood cover with strong-radius $\tO(D)$ and quality $q = \tO(1)$. 
The algorithm needs access to a $(1+\eps)$-approximate tree-like distance oracle $\fO$ up to distance $\tO(D)$. It needs $\tO(1)$ aggregations along outputs of $\fO$ and $\tO(1)$ global aggregations. 
\end{corollary}
\begin{proof}
We repeat \cref{cor:separated_padded_clustering} $O(\log n)$ times, in the $i$-th step we get clustering $\fC_i$. 
Each time we set $\delta_\Coref{cor:separated_padded_clustering} = 1/2, D_\Coref{cor:separated_padded_clustering} = D$. 
At the beginning, we set $\mu_{1, \Coref{cor:separated_padded_clustering}}$ to be an identity function and in the $i$-th call we set $\mu_{i, \Coref{cor:separated_padded_clustering}}(u) = 0$ if $u$ was happy in at least one clustering $\fC_1, \fC_2, \dots, \fC_{i-1}$. Otherwise, $\mu_{i, \Coref{cor:separated_padded_clustering}}(u) = 1$. 
As we have $\mu_{i+1, \Coref{cor:separated_padded_clustering}}(V(G)) \le \mu_{i, \Coref{cor:separated_padded_clustering}}(V(G))/2$, after $O(\log n)$ iterations, each node was happy in at least one clustering. 
\end{proof}

Above two are essentially the results from the sssp paper

\begin{corollary}[ball growing with cutting edges]
Let $G$ be a weighted graph and $D, \delta > 0$ parameters. Then there is an algorithm constructing a partition $\fC$ with strong-radius $\tO(D/\delta)$ such that the number of unclustered edges is bounded by $\tO(\delta \sum_{e \in E(G)} w(e) / D)$.
The algorithm needs access to a $(1+\eps)$-approximate tree-like distance oracle $\fO$ up to distance $\tO(D)$. It needs $\tO(1)$ aggregations along outputs of $\fO$ and $\tO(1)$ global aggregations. 
\end{corollary}
\begin{proof}
Consider the graph $G'$ that we get by subdividing each edge of $G$. 
That is, we have $V(G') = V(G) \cup E(G)$ and for every $e = \{u,v\} \in E(G)$ we have an edge $\{u, e\}$ in $E(G')$ of weight $w(e)/2$. Note that for any $u,v \in V(G)$ we have $d_G(u, v) = d_{G'}(u,v)$. 
Moreover, we define a weight function $\mu$ on $G$ as follows: For each $u \in V(G)$ we set $\mu(u) = 0$ and for each $e \in E(G)$ we set $\mu(e) = 1$. 

Next, we run \cref{thm:steroids} with $G_\Tref{thm:steroids} = G', S_\Tref{thm:steroids} = V(G), R_\Tref{thm:steroids} = 0, D_\Tref{thm:steroids} = D, \delta_\Tref{thm:steroids} = \delta$. 
The $(1+\eps)$-distance oracle on $G'$ is implemented as follows \todo{either fill in or state differently}. 
Let $\fC' = \fC_\Tref{thm:steroids}$. For each $C' \in \fC'$ we define a cluster $C \in V(G)$ by setting for any $u \in V(G)$ that $u \in C$ if and only if $u \in C'$. This defines a partition $\fC$ of $G$. 

The strong-radius of each cluster $C$ is upper bounded by the strong-radius of the respective cluster $C'$, that is the partition $\fC$ is $\tO(1)$-strong radius. 
Note that the total weight of miserable nodes $M' = M_\Tref{thm:steroids}$ in $\fC'$ is bounded by $\mu(M') = \tO(\delta \sum_{e \in E(G)} w(e)/(2D))$. 
Since every edge $e \in E(G)$ that is unclustered in $\fC$ is a miserable node in $\fC'$, we also get that the number of unclustered edges is bounded by $\tO(\delta \sum_{e \in E(G)} w(e)/D)$, as needed. 
\end{proof}


\begin{corollary}[ball growing with cutting edges and terminals]
write main theorem in term edges, i.e., complete clustering with terminals S covering radius $D_S$, get clustering with radius $(1 + eps)D_S + D'$ and cut $polylog n sum_e l_e/D'$ edges.
assume $\tO(1)$ aggregate roundsin weighted and $\tO(D)$ congest in unweighted graphs? 
\end{corollary}
\begin{proof}

subdivision+ $r_e=l(e)/2$
\end{proof}

above corolaries have also randomized versions. 


\subsection{deterministic and probabilistic tree embeddings}

\begin{definition}[2-HST, cf. Definition 7, Bartal 96]
A $2$-hierarchically well-separated tree ($2$-HST) is defined as a rooted weighted tree with the following properties:
\begin{enumerate}
    \item The edge weight from any node to each of its children is the same.
    \item The edge weights along any path from the root to a leaf are decreasing by a factor of at least $2$.
\end{enumerate}
\end{definition}



\begin{theorem}[\cite{becker_emek_lenzen2020blurry_ball_growing}]
\label{thm:bartal_rand}
There exists an algorithm that computes a $2$-HST $T$ coming from a distribution $\mathcal{T}$ such that $V(G) \subseteq V(T)$ and for every edge $e = \{u,v\} \in E(G)$, we have

\[\E_{T \sim \mathcal{T}} [d_T(u,v)] = \tilde{O}(1) \ell(u,v).\]

The algorithm runs in .
\end{theorem}


One needs to define a deterministic analog to bartal rand
The most is that the deterministic algorithm outputs a complete description of the distribution $\mathcal{T}$. However, one can show that on a cycle one of the edges is stretched by a $\Omega(n)$ factor. This gives a lower bound of as in the cycle worst-case stretch can be $\Omega(n/\log^2(n))$ on the support of the distribution. Hence, an overall size of $\Omega(n^2/\log^2(n))$ and therefore we cannot hope for efficient algorithms based on this.
Instead, the right deterministic analog of is the following.

https://dl.acm.org/doi/pdf/10.5555/1109557.1109665

\todo{For the general clustering result, should we add that the output partition does not depend on the input radii?}

\begin{theorem}
There exists an algorithm that computes a collection $T_1,T_2, \ldots, T_k$ of $2$-HST and a collection of sets $vgood_1$for $k = O(\log n)$ together with a co
\end{theorem}
\begin{proof}

\end{proof}

We also prove a deterministic analog: log n   partial tree embeddings such that 1 / 1 polylog n fraction of nodes are happy in each tree, built by multiplicative weightes
This results follows from well-separated clustering. Probably we should reprove it, but it has low priority 

deterministic h hop bounded analog of the partial tree embedding is proved the same way as above result, we just need to add some blabla about how the oracle runs in h steps as it is bellman/ford. Hence running time is $\tO(D + h)$ . We in general use the mixture metric $w_i(e) = 1 + l(e)/2^i$ and look up to distance $h$ in this metric. 

Finally, the last result we will prove is deterministic bartal (frt) analog which minimizes weighted sum of stretched edge length instead of saying that 0.99 of nodes are happy. 
This might follow from setting cost of e = weight * length in subdivided graph


\subsection{corolaries of tree embeddings}

steiner trees , h-hop steiner tree
do not need to be proven, just state and cite





==> img/old/old.tex <==

\subsection{Binary Search}

\begin{lemma}
\label{lem:binsearch}
Let $G$ be a weighted graph, $U \subseteq V(G)$ and $D, \eps > 0$ parameters. We assume access to an $(1+\eps)$-approximate tree-like oracle $\fO$. 
Then, there is a distributed algorithm that returns
\begin{enumerate}
    \item A set $W \subseteq V(G) \setminus U$ 
    \item A rooted forest $T_W, V(T_W) \subseteq W \cup U$ such that the roots nodes of $T_W$ are the nodes of $U$
    \item A set $M \subseteq V(G)$ containing all miserable nodes. Here, we say that a node $v \in V(G)$ is miserable if $v \in W \cup U$ and $B_G(v, r_v) \not\subseteq W \cup U$ or $v \in V(G) \setminus (W \cup U)$ and $B_G(v, r_v) \not\subseteq V(G) \setminus (W \cup U)$. 
\end{enumerate}

The output has the following properties. 

\begin{enumerate}
    \item For each component $T$ of $T_W$ we have $\rad(T) \le D + O(\eps D)$. 
    \item $\mu(M) \le O(\log n \cdot \sum_{u \in V(G)} \mu(u) r_u / D)$. 
\end{enumerate}
\end{lemma}

\begin{proof}
It will be $t = O(\log n)$ step binary search. 

At the $i$-th step we have the set of white nodes $U_i$ and the set of black nodes $B_i$. 
We have $U = U_0 \subseteq U_1 \subseteq \dots \subseteq U_t = W \cup U$ is the output and $\emptyset = B_0 \subseteq B_1 \subseteq \dots \subseteq B_t$.  
In the $i$-th step, we run an oracle $\fO$ on $G[V(G) \setminus B_i]$ from $U_i$ up to distance $(1+\eps)D_i$ for $D_i = D \cdot ((1-\eps)/2)^i$. 

At the beginning, we run $\fO$ up to distance $2D_0$. We make everything in distance greater than $(1+\eps)D_0$ black, i.e., in $B_0$. 

Every node $u \in V(G)$ is either satisfied or unsatisfied. If it is unsatisfied, it has an interval $I_{u, i} = [\td_i(u) - l_{u,i}, \td_i(u) + r_{u,i})$. Formally, we have $\emptyset = S_0 \subseteq S_1 \subseteq \dots \subseteq S_t$ and we set $M = V(G) \setminus S_t$. 

At the beginning every node is unsatisfied. We have $I_{u, 0} = [\td_0(u) - r_u, \td_0(u) + r_u)$, i.e., $l_{u,i} = r_{u,i}  = r_u$. The exception is the black nodes, for them  $I_{u, 0} = [\td_0(u) - r_u - \eps D, \td_0(u))$. 

We define
\[
\zeta_i = \frac{\sum_{u \in V(G) \setminus S_i} |I_{u, i} \cap [0, D_i)|}{ D_i }
\]

At the beginning, we have $\zeta_0 \le \frac{\sum_{u \in V(G)} |I_{u, 0}|}{D} \le \frac{\sum_{u \in V(G)} O(r_u)}{D}$. 

We preserve the following invariants. 

\begin{enumerate}
    \item $\zeta_{i} \le (1+\eps)^i \zeta_0$
    \item $U_i$ is $D_i$-ruling set in $G[V(G) \setminus B_i]$.  
    \item If $u \in S_i$, either $u \in U_i$ and $B(u, r_u) \subseteq U_i$ or $u \in B_i$ and $B(u, r_u) \subseteq B_i$. 
\end{enumerate}

At the beginning of the algorithm, both invariants hold. 
The algorithm does the following. 
Let us define $I'_{u, i} = I_{u,i}$ if $[D_i/2 - \eps D_i, D_i/2 + \eps D_i) \not\subseteq I_{u, i}$ and $I'_{u, i} = [\td_i(u) - l_{u,i} - \eps D_i, \td_i(u) + r_{u, i} + \eps D_i)$ otherwise. 

In the $i$-th step, we run $\fO$ to find $\td_i(U_i, \cdot)$. By the ruling invariant, all grey nodes have $\td_i(U_i, v) \le (1+\eps)D_i$. 
We compute two values
\[
\zeta_{l} = \frac{\sum_{u \in V(G) \setminus S_i} |I'_{u,i} \cap [0, (1-\eps)D/2]| }{ (1-\eps)D/2}
\]
and
\[
\zeta_{r} = \frac{ \sum_{u \in V(G) \setminus S_i} |I'_{u,i} \cap [(1+\eps)D/2, D]| }{ (1-\eps)D/2}
\]

If $\zeta_l \le \zeta_r$, we mark all nodes in $\tT_i$ with $\td_i(u) \ge D_i/2 - \eps D_i$ as black. 
Otherwise, we mark all nodes in $\tT_i$ with $\td_i(u) \le D_i/2 + \eps D_i$ as white. 

If $u$ got white and $I_{u,i}$ is not intersecting $[D_i/2, D_i)$, then we make $u$ satisfied (and make its interval empty from now on). 
Otherwise, we set $I_{u, i+1} = [0, \td(u) + r'_{u,i} - D/2 + \eps D)$. 

If $u$ got black and $I_{u,i}$ is not intersecting $[0, D_i/2)$, then we make $u$ satisfied (and make its interval empty from now on). 
Otherwise, we set $l_{u, i+1} = l'_{u, i}, r_{u, i+1} = r'_{u,i}$. 


\begin{claim}
The third invariant holds
\end{claim}
\begin{proof}
We will prove by induction that whenever $u \in U_i \cup B_i$ and we have another $v \in B(u, r_u)$, then $\td_j(v) \in I_u$ for $j \ge i$. 
Let $i$ be the first 

\end{proof}

\begin{claim}
$\zeta_{i+1} \le (1+\eps)\zeta_i$
\end{claim}


We finish the process when $D_i = R_i - L_i = O(1)$ and color every remaining node white. 
Since $|I_{u,i} \cap [L_i, R_i) = O(1)$, $\zeta$ is just the number of intervals intersecting $[L_i, R_i)$. We put all nodes $u$ with nontrivial $I_u$ to $M$. Due to zeta invariant, their number is what it should be. 


\end{proof}












\begin{comment}
\paragraph{OLD!}
For each $\fA \in \{\fR,\fB\}$, we run the oracle $\fO$ with $\eps_\fO = \eps$ to compute $(1+\eps)$-approximate tree-like distances from $U_i^\fA$ in $G[V_i^\fU] = H_i[V_i^\fU]$. 
We get a pair $(\hd_i^\fA(U_i^\fA, \cdot), \hT_i^\fA)$. 

We also use a shorthand $\hd_i^\fA(u) = \hd_i^\fA(U_i^\fA, u)$. \todo{drop?}

Next, for each $\fA \in \{\fR,\fB\}$ we will find a threshold $0 \le \tau_i^\fA \le D$ and define $W_i^\fA$ as the set of all nodes $u \in V_i^\fU$ such that $\hd_i^\fA(U_i^\fA, u) \le \tau_i^\fA$. 
The threshold $\tau_i^\fA$ is found by binary search to ensure that the total weight of nodes $u \in V_i^\fU$ such that $\hd_i^\fA(u) - \tau_i^\fA \le 2r_u$ is bounded by $O(\sum_{u \in V_i^\fU} \mu(u) r_u / D)$. 

More concretely, at the beginning we set $\tau_{low} = 0$ and $\tau_{high} = D$. 
%We also keep a variable $\tau_{mid}$. 
For each node $u \in V_i^\fU$ we define an interval $I_u = [\hd_i^\fA(u) - 2r_u, \hd_i^\fA(u) + 2r_u)$. 
Let 
\[
\xi(\tau_{low}, \tau_{high}) = \frac{\sum_{u \in V_i^\fU} \mu(u) \cdot |I_u \cap [\tau_{low}, \tau_{high}) |}{\tau_{high} - \tau_{low}}.
\]
At the beginning, we have $\xi(\tau_{low}, \tau_{high}) = \sum_{u \in V_i^\fU} \mu(u) |I_u| /D =  4\sum_{u \in V_i^\fU} \mu(u) r_u/D$. 
In each iteration of the binary search, we set $\tau_{mid} = (\tau_{low} + \tau_{high}) / 2$ and use a global aggregation to compute the value of $\xi(\tau_{low}, \tau_{mid})$ and $\xi(\tau_{mid}, \tau_{high})$. 
Clearly we have $\min( \xi(\tau_{low}, \tau_{mid}), \xi(\tau_{mid}, \tau_{high}) ) \le \xi(\tau_{low}, \tau_{high})$. 
If $\xi(\tau_{low}, \tau_{mid}) \le \xi(\tau_{low}, \tau_{high})$, we set $\tau'_{low} = \tau_{low}$ and $\tau'_{high} = \tau_{mid}$ in the binary search, otherwise we set $\tau'_{low} = \tau_{mid}$ and $\tau'_{high} = \tau_{high}$. 
After $O(\log n)$ iterations of the binary search, we get $\tau_i^\fA = \tau_{low} = \tau_{high}$. Let $M_i^\fA$ be the set of  such that nodes $u \in V_i^\fU$ such that $I_u \cap \{\tau_i^\fA\} \not= \emptyset$. By above reasoning, we have
\begin{align}
\label{steroids:eq:boundary}
\mu(M_i^\fA) \le 4 \sum_{u \in V_i^\fU} \mu(u) r_u /D.  
\end{align}


We communicate the value of $\tau_i^\fA$ to the whole graph $G$ in a global aggregation round and set $W_i^\fA$ to be the set of nodes in $V_i^\fU$ such that $\hd_i^\fA(u) \le \tau_i^\fA$. 
Any node $w \in W_i^\fA$ learns the value $\bd(u)$ of the root $u \in U_i^\fA$ of its tree in $\tT_i^\fA$ and sets $\bd(w) = \bd(u) + \hd_i^\fA(w)$ (we prove in \cref{steroids:cl:W} that $W_i^\fR \cap W_i^\fB = \emptyset$, hence this is well-defined). 

%Next, we repeat the binary search procedure for blue nodes in the same manner to get sets $M_i^B$ and $W_i^\fB$. 

%First, we compute  distances from $U_i^\fB$ in $G \upharpoonright (V(G) \setminus (V_i^\fR \cup U_i^\fR \cup W_i^\fR)$. 
%We get a pair $(\hd_i^B(U_i^\fB, \cdot), \hT_i^B)$.
%Next, we find a threshold $0 \le \tau_i^B \le D$ and define $W_i^\fB$ as the set of all nodes $u \in V_i^\fU$ such that $\hd_i^B(U_i^\fB, u) \le \tau_i^B$ and the number of nodes with ... is at most $\sum_{u \in V(G)} \mu(u) 4r_u /D$. 
 \end{comment}












\paragraph{OLD}
Recall that a node $u \in V_i^\fA$ for $\fA \in \{\fR,\fB,\fU\}$ is miserable if $B_G(u, r_u) \not\subseteq V_i^\fA$. 
First, we prove by induction that $M_i$ contains all miserable nodes in the $i$-th phase. It holds for $i=0$, suppose it holds for some $i$. 

Let $u \in V_i^\fR \cup V_i^\fB$ be such that $u$ is miserable in the $(i+1)$-th step. It was also miserable in the $i$-th step, since $V_{i}^A \subseteq V_{i+1}^\fA$ for $\fA \in \{\fR,\fB\}$. 
Hence, by induction we get $u \in M_i \subseteq M_{i+1}$ as needed. 

Next, let $u \in V_i^\fU$ be such that $u$ is miserable in the $i+1$-th step. If $u$ was also miserable in the $i$-th step, by induction $u \in M_i \subseteq M_{i+1}$ and we are done. Hence, assume the opposite is true, i.e., $B(u, r_u) \subseteq V_i^\fU$. 
Recall that by the definition of miserability we have that either $u \in V_{i+1}^\fU$ and $B(u, r_u) \not\subseteq V_{i+1}^\fU$, or $u \in U_i^\fA \cup W_i^\fA$ but $B(u, r_u) \not\subseteq V_{i+1}^\fA =  U_i^\fA \cup W_i^\fA \cup V_i^\fA$, for some $\fA \in \{\fR,\fB\}$. 

First, consider the case $u \in V_{i+1}^\fU$. 
The above facts imply that there is some node $v$ with  $d_{G[V_i^\fU]}(u,v) \le r_u$ such that  $v \in V_i^\fU \setminus V_{i+1}^\fU$, hence $v \in U_i^\fA \cup W_i^\fA$ for some $\fA \in \{\fR,\fB\}$. 
We have
\begin{align*}
\hd_i(u) 
&\le \hd_i(v) + (1+\eps) d_{G[V_i^\fU]}(u,v) && \text{$\hT$ is smooth} \\
&\le \tau_i^\fA + 2r_u && \text{$v \in U_i^\fA \cup W_i^\fA$} \\
\end{align*}
Hence, for the interval $I_u = [\hd_i^\fA(v) - 2r_v, \hd_i^\fA(v) + 2r_v)$ from the binary search in part 2 of the $i$-th phase we have $I_u \cap \{\tau_i^\fA\}$ is nonempty, hence $u \in M_i^\fA \subseteq M_{i+1}$, as needed. 

Next, consider the case $u \in U_i^\fA \cup W_i^\fA$, but $B(u, r_u) \not\subseteq V_{i+1}^\fA$, for some $\fA \in \{\fR,\fB\}$. 
Above facts imply existence of a node $v$ with $d_{G[V_i^\fU]}(u,v) \le r_u$ such that $v \in V_i^\fU \setminus \left( U_i^\fR \cup W_i^\fR \cup U_i^\fB \cup W_i^\fB \right)$. 
We have
\begin{align*}
\hd_i(u) 
&\ge \hd_i(v) - (1+\eps) d_{G[V_i^\fU]}(u,v) && \text{$\hT$ is smooth} \\
&\ge \tau_i^\fA - 2r_u && \text{$v \not\in U_i^\fA \cup W_i^\fA$} \\
\end{align*}
Hence, analogously to the previous case, $u \in M_i^\fA \subseteq M_{i+1}$. 

Finally, we bound the size of the set $M_i$. Recall that we have $\mu(M_i^\fA) \le 4 \sum_{u \in V(G)} \mu(u) r_u /D $ by \cref{steroids:eq:boundary}. Hence, 
\begin{align}
    \mu(M_i) \le 8i \cdot \sum_{u \in V(G)} \mu(u) r_u /D. 
\end{align}
\todo{maybe it is not necessary to consider $r_u > D$ separately?}




































































\begin{proof}
We will first assume that besides regular \congest message passing rounds we also have access to some steps where we can compute certain global aggregate operations. 
In the end, we lift this requirement by first constructing another low diameter clustering. 
This larger clustering is used to implement the global operations. 

We first assume that the algorithm has also access to certain global opeartions beside classical \congest. Then, we show how to implement these global operations using network decomposition. 

We use the following algorithm that has $t = 1 + \log_2 n$ phases. 
We start with the input graph $G = G_0$ and gradually remove nodes from it, together with incident edges, to build a sequence $G_0 \supseteq G_1 \supseteq \dots \supseteq G_t = \emptyset$. During the procedure, we build a clustering $\fC_0 \subseteq \fC_1 \subseteq \dots \subseteq \fC_t$. Each cluster in $\fC_i$ has diameter at most $10 \Dldd(n,k)$. 
For the final cluster $\fC_t = \fC$ we will have $V(\fC) = V(G)$, i.e., it is a partition. 
The $i$-th step of the algorithm has two parts. 

First, we use \cref{thm:strong_clustering} with $k_\Tref{thm:strong_clustering} = 10k$ to build a strong-diameter clustering $\fC'_i$ of $G_i$ that clusters at least $|V(G_i)|/2$ nodes. 

Next, we implement the following procedure. 
We consider the current clustering $\fC'_i$ and compute the number of nodes of $G[V(G) \setminus \fC'_i]$ neighboring with $\fC'_i$. If their number is at least $|\fC'_i|/k$, we grow each cluster in  $\fC'_i$ by adding its neighborhood to it. 
We continue this growing procedure until $\fC'_i$ stops growing. Then, we set $\fC_{i+1} = \fC_i \cup \fC'_i$ and $G_{i+1} = G_i \setminus G_i[\fC'_i]$.

This finishes the description of the algorithm. It remains to be argued that its output has the desired properties and that it can be implemented in the \congest model. We do this next. 



\begin{claim}
\label{cl:strong}
For each $i$, the growing process of the clustering $\fC'_i$ in the second part of the $i$-th phase finishes after at most $4k$ rounds. 
Hence, for any $C_1, C_2 \in \fC_i$ we have that $C_1$ and $C_2$ are not neighboring; in particular $C_1 \cap C_2 = \emptyset$. 
\end{claim}
\begin{proof}
In each step of the growing process in the second part of the $i$-th phase, the size of the growing cluster $C \in \fC_i'$ grows multiplicatively by a factor of $1 + 1/k$. 
Hence, after $10k$ rounds, the size of $\fC_i'$ is at least
\[
n/2 \cdot (1 + 1/k)^{4k} 
\ge n \cdot \frac12 \cdot 2^4
> n. 
\]
a contradiction. As we chose $k_\Tref{thm:strong_clustering} = 10k$, we get for any $C_1 \not= C_2 \in \fC'_i$ that $d(C_1, C_2) \ge 10k - 2 \cdot 4k > 0$, hence in particular $C_1 \cap C_2 = \emptyset$ as needed. 
\end{proof}

\begin{claim}
\label{cl:diam}
We have for each $i$ that
\[
\hopdiam(\fC_i) \le \Dldd(n, 10k) + 10k. 
\]
\end{claim}
\begin{proof}
Note that each cluster $C \in \fC_i$ starts, by definition, with diameter at most $\Dldd(n, 10k)$. Next, note that in each step, the cluster diameter can only increase additively only by $2$. 
Together with \cref{cl:strong} this implies that at the end of the $i$-th phase, we have
\begin{align*}
\hopdiam(C) 
\le \Dldd(n, 10k) + 2 \cdot 4k 
\le \Dldd(n, 10k) + 10k
\end{align*}
as needed. 
\end{proof}

\begin{claim}
\label{cl:partition}
$\fC_t$ is a partition of $G$. 
\end{claim}
\begin{proof}
Note that $|V(G_i)| \le |V(G_{i-1})| / 2$ by the definition of a low diameter clustering in \cref{def:low_diameter_clustering}. 
Hence, for $t = \log_2 n + 1$ we have $|V(G_t)| \le n/2^{\log_2 n + 1} < 1$, i.e., $G_t$ is empty. 
\end{proof}

\begin{claim}
\label{cl:edges}
We have $|E(\pi_\fC(G))| \le n/k$. 
\end{claim}
\begin{proof}
Consider any node $\pi_\fC(C) \in \pi_\fC(G)$ that corresponds to some cluster $C \in \fC$. Let $i$ be the phase when the cluster $C$ was created. 

By construction, when $C$ stopped growing, it was the case that that it neighbored with at most $|C| /k$ nodes in $G_i$. 
This implies that number of edges in $\pi_\fC(G)$ between $\pi_\fC(C)$ and clusters $C'$ created in some phase $j > i'$ is at most $|C| /k$. 
The number of edges in $\pi_\fC(G)$ between $\pi_\fC(C)$ and clusters $C'$ created in phase $i$ is equal to zero by \cref{cl:strong}. 

Above reasoning implies that $|E(\pi_\fC(G))| \le \sum_{C \in \fC} |C|/k$. As all clusters are disjoint by \cref{cl:strong}, we get $|E(\pi_\fC(G))| \le |\bigcup_{C \in \fC} C|/k = n/k$. 
\end{proof}

Above claims imply that the clustering $\fC$ has the desired properties. It remains to argue about its round complexity. 

\begin{claim}
\label{cl:time}
The algorithm can be implemented in $O(\log n) \cdot \left( \Tldd(n, 10k) + k\Dldd(n,10k) \right)$ deterministic \congest rounds. 
\end{claim}
\begin{proof}

So far, we introduced the algorithm as a one relying on global coordination: in each growing step, the whole graph $G_i$ needs to coordinate whether the clusters in it grow or not. 
This requirement can be lifted by the following application of the low diameter clustering. 

We show how to implement a slightly different variant of the presented algorithm where in each phase the clustering $\fC'_i$ contain only $|V(G_i)|/4$ nodes, not $|V(G_i)|/2$. One can set the number of phases $t = 1 + \log_4 n$ instead of $t = 1 + \log_2 n$ and the analysis above remains true. 

Each phase in the new variant of the algorithm starts by computing a low diameter clustering $\tfC_i$ with separation $10k$. We have 
\begin{align}
    \label{eq:bob}
    |\bigcup_{\tC \in \tfC_i} \tC| \ge |V(G_i)/2|. 
\end{align}
Next, we run the same algorithm as described, but it is run separately in each cluster $\tC$. 
That is, each cluster $\tC$ first computes a low diameter clustering of it and then proceeds with at most $4k$ growing steps by \cref{cl:strong}.  

The first part of the algorithm, computing a low diameter decomposition inside each cluster, can be implemented simply by one low diameter clustering computation on the subgraph $G_i[\bigcup \tfC_i]$ of $G_i$. 

Each step in the second part of the algorithm can be implemented in $O(\Dldd(n, 10k))$ \congest rounds, as we can aggregate the relevant information in the root of each cluster of $\tfC$. 
The final clustering $\fC'_i$ we compute this way has the property that $|\bigcup_{C \in \fC'_i} C| \ge |\bigcup_{\tC \in \tfC_i} \tC|/2 \ge |V(G_i)|/4$ where the first inequality follows from the fact that we build the low diameter clustering in each $\tC \in \tfC_i$ and the second is by \cref{eq:bob}. 
The fact that $\tfC_i$ is $10k$-separated implies that $\fC'_i$ is $10k$-separated, too. 
This implies that this version of the algorithm is still correct. 

Moreover, each phase of it can be implemented in $\Tldd(n, 10k) + O(k) \cdot \Dldd(n,10k)$ rounds. This implies that the round complexity of the algorithm is 
\[
O(\log n) \cdot \left( \Tldd(n, 10k) + k\Dldd(n,10k) \right),
\]
as needed. 
\end{proof}
\end{proof}


We are now ready to prove \cref{thm:unweighted_spanner} that we restate here for convenience. 

\unweighted*

\begin{proof}
We apply \cref{lem:unweighted_contraction} to give us a graph $G' = G/F = \pi_F(G)$ where $F$ is a spanning forest of a partition $\fC$ of $G$. We define $H$ as follows. We include all edges of $F$. 
Next, for each edge $e \in E(G')$, we take an arbitrary edge in $\pi^{-1}_F(e)$ and add it to $H$. This finishes the construction. 

\begin{claim}
\label{cl:unweighted_edges}
$|E(H)| \le n + n/k$. 
\end{claim}
\begin{proof}
We have $|E(F)| \le n$ since $F$ is a forest. Next, we added at most $|E(G')| \le n/k$ edges due to the guarantee of \cref{lem:unweighted_contraction}. 
\end{proof}

\begin{claim}
\label{cl:unweighted_diam}
$H$ is a $3\hopdiam(F) = O(k \log^3 n)$ spanner. 
\end{claim}
\begin{proof}
Consider any two nodes $u, v$ and a shortest path $P$ between them in $G$. 
We describe a sequence of edges $P' \subseteq H$ between $u$ and $v$ in $H$ such that
\[
d_{P'}(u, v) \le 3\hopdiam(F) d_P(u, v). 
\]

This is done as follows. Consider any edge $\{u', v'\}$ in $P'$. 

There are two possibilities. Either $u', v'$ belong to the same cluster $C \in \fC$. 
In that case, replace $\{u', v'\}$ by the unique path from $u'$ to $v'$ in $C$. This path has length at most $\hopdiam(C) \le \hopdiam(F)$. 

Other possibility is that $u' \in C_1$ while $v' \in C_2 \not= C_1$. 
In that case, the existence of $e$ implies that $H$ contains an edge $e' = \{x, y\}$ (possibly $e' = e$) with $x \in C_1, y \in C_2$. 
Replace $\{u', v'\}$ by the unique path connecting $u'$ with $x$ in $C_1$, followed by the edge $e'$, followed by the unique path from $y$ to $v'$. The length of this path is at most 
\[
\hopdiam(C_1) + 1 + \hopdiam(C_2) 
\le 3\hopdiam(F). 
\]
This finishes the proof. 
\end{proof}

\begin{claim}
\label{cl:unweighted_time}
The algorithm can be implemented in $O(\snd(n, k \log n) \cdot \log n + k^2 \log^6 n)$ \congest rounds. \todo{fix complexity}
\end{claim}
\begin{proof}
The algorithm invokes \cref{lem:unweighted_contraction} with round complexity $O(\snd(n, k \log n) \cdot \log n + k^2 \log^6 n)$. 
After that, we need $O(\hopdiam(F)) = O(k \log^4 n)$ rounds to build the spanner. 
\end{proof}

The proof follows from \cref{cl:unweighted_edges,cl:unweighted_diam,cl:unweighted_time}. 
\end{proof}



\begin{proof}
We use the following algorithm. Every cluster $C$ starts with a unique $b = O(\log n)$-bit identifier. It can be e.g. an  identifier of an arbitrary node in it. 

At the beginning of the algorithm, all clusters are \emph{alive}. During the algorithm some clusters stop being alive. 

The algorithm has $b = O(\log n)$ phases. 

%In the $i$-th phase, we say that an alive cluster is \emph{active} if the $i$-th bit of its identifier is $1$; otherwise it is not active. 

During the $i$-th phase, we run for $2k$ steps the following BFS-like procedure. 
We preserve a set of \emph{untouched, open} and \emph{closed} clusters. 
At the beginning, every alive cluster such that the $i$-th bit of its identifier is $1$ is open. All other clusters are untouched. 

Each open cluster knows a number of a \emph{closing step} $j$. The closing step of each cluster $C$ open at the beginning is $\hopdiam(C)$.
At the step $j$, the open cluster becomes closed and opens all of its neighboring untouched clusters. 
In particular, every neighboring cluster $C$ opens and sets its closing step to be $j + \hopdiam(C)$. 

After $k$ steps of this procedure, we mark all open and closed clusters such that the $i$-th bit of their identifier is $0$, as not alive. 

After all $b$ phases of the algorithm are finished, we run the same BFS-like procedure from every alive cluster, until all clusters are closed. The clusters reached from each alive $C$ form a new connected cluster $C'$. Partition $\fC'$ to these new clusters is the output of the algorithm. 

This finishes the description of the algorithm. 

Let us mention a different way of viewing the BFS procedure. It corresponds to a BFS in the following graph $G'$. In $G'$, every cluster $C$ corresponds to two nodes, an input an output node. There is an oriented edge from the input one to the output one of length $\hopdiam(C)$. There is an oriented edge of length $1$ between an output node of $C$ and an input node of $C'$ if and only if $C$ and $C'$ neighbor in $G$. \todo{maybe we can just say this and directly reduce to ruling set?}

Next, we argue about its correctness and round complexity. 

\begin{claim}
\label{cl:ruling}
In step $i$, every inactive cluster is at distance at most $6i \cdot k$ from an active cluster. 
In particular, at the end of the algorithm, every cluster has distance $O(k\log n)$ to an active cluster. 
\end{claim}
\begin{proof}
It holds for $i = 0$, assume it holds for some $i$ and we prove it for $i+1$. 

First, note that during the BFS procedure in the $i+1$ phase, a cluster $C$ becomes open in a step $j$ only if its distance to an initially open cluster is at most $j$. This follows from a standard BFS analysis together with the fact that each cluster $C$ waits for $\hopdiam(C)$ time before it opens its neighbors. 

Hence, every cluster $C$ that is closed at the end of the procedure has a distance at most $k$ to some initially open cluster $C'$ that stays alive after the $i+1$-th phase is over. If $C$ is open at the end of the procedure, the same holds but the distance to $C'$ is at most $2k + \diam(C) \le 3k$. 

Hence, for every cluster $C_0$ that is inactive after step $i$, we can find by induction a cluster $C$ that is active after step $i$ and $d(C_0, C) \le 6ik$. Next, above argument shows that we can find a $C'$ such that $C'$ is active after phase $i+1$ and $d(C, C') \le 3k$. Hence, 
\[
d(C_0, C') \le d(C_0, C) + \hopdiam(C) + d(C, C') \le 6(i+1)k
\]
as needed. 
\end{proof}

Note that (an argument similar to) \cref{cl:ruling} implies that for each $C' \in \fC'$ we have $\hopdiam(C') = O(k \log n)$. 

\begin{claim}
Every cluster $C' \in \fC'$ has $|C'| \ge k$. 
\end{claim}
\begin{proof}
If there is just one cluster $C'$ in $\fC'$, it holds by our assumption $|V(G)| \ge k$. Otherwise, let $C' \in \fC'$ and $C \in \fC$ be the unique alive cluster such that $C \subseteq C'$. 
Note that if we start BFS from the input cluster of $C$, we arrive to another alive cluster only after $2k$ steps. This means that everything we reach from $C$ after at most $k$ steps is in $C'$. Hence, $|C'| \ge k$ as needed. 
\end{proof}

\begin{claim}
\label{cl:round_complexity}
The algorithm can be implemented such that it finishes after $O(k \log n)$ rounds. 
\end{claim}
\begin{proof}
We show that the BFS procedure in every phase can be implemented in $O(k)$ \congest rounds. 
To see this, note that whenever a cluster $C$ is open at some node $u \in C$, it should close and open its neighbors only in $\diam(C)$ rounds. 
In this many rounds, $u$ can flood $C$ with the information of its closing step. There can be possibly several nodes trying to flood $C$ with this information as $C$ can be open at different nodes around the same time. Whenever several floods arrive to the same node, it chooses the earliest closing time. We omit details. 
\end{proof}
\end{proof}








































\begin{comment}
\newpage
We are now ready to give a distributed algorithm building the promised partition of any unweighted graph. 
The algorithm assumes that the graph $G$ contains edges of only $b$ different weights. This is not a strong assumption -- before we apply this result, we first discretize the weights of the given graph so that $b = O(\log n)$. 

\begin{lemma}
\label{lem:bernard_contraction}
Suppose we are given a connected weighted graph $G$ with $b$ different edge-weights $w_0 < \dots < w_{b-1}$, and a parameter $k < V(G) = n$. 
There is a deterministic \congest algorithm that, outputs a clustering $\fC$ such that
\begin{enumerate}
    \item $\fC$ has the pretty property. 
    \item each $C \in \fC$ satisfies $|C| \ge k$
    \item For every $C \in \fC$ we have the hop diameter $\hopdiam(C) = O(k \log n)$
\end{enumerate}
in $\poly (bk \log n)$ \congest rounds. 
\end{lemma}

\begin{proof}
Let $w_0 < w_1 < w_2 < \dots < w_{b-1}$ be the different edge-weights in $G$. 
The algorithm has $b = O(\log n)$ phases. 
In the $i$-th phase, we have a remainder graph $G_i$ with edge-weights and node-weights.
At the beginning, $G_0 = G$, with all node weights set to $1$. 
At the end, we have $G_t = \emptyset$. 

%During the construction, we build a strong clustering $\emptyset = \fC_0 \subseteq \fC_1 \subseteq \dots \subseteq \fC_b = \fC$, together with its spanning forest $F$. The final clustering $\fC$ is a partition (it covers all nodes of $G$). 

During the construction, we build a spanning forest $\emptyset = F_0 \subseteq F_1 \subseteq \dots \subseteq F_b = F$. 
Connected components of each $F_i$ are moreover split to the \emph{big} ones, $F_i^{\ge k}$, that contain at least $k$ nodes and \emph{small} ones, $F_i^{< k}$, that contain less than $k$ nodes. 
%In the end, we have $V(F_i^{\ge k}) = V(G)$. 
During the algorithm, we define $G_i$ and a contraction $\pi_i$ as 
\[
G_i = \pi_i(G) = G / F_i. 
\]
Moreover, we define $G_i^{\ge k} = G_i[F_i^{\ge k} / F_i^{\ge k}]$ and $G_i^{< k} = G_i[F_i^{< k} / F_i^{< k}]$. That is, $G_i^{\ge k}$ is the subgraph of $G_i$ induced by nodes of $G_i$ that correspond to components of $F_i$ of size at least $k$. 

Our construction will preserve the following invariants. 

\begin{enumerate}
    \item If an edge $e$ of $G_i$ has weight smaller than $w_i$, then $e \in G_i^{\ge k}$.
    \item $F_i$ has the pretty property. 
    \item $\hopdiam(F_i) = O(k \log n) + i \cdot O(k)$
%    \item Every connected component of $G_i$ has its node-weighted size at least $k$. 
\end{enumerate}

We now describe the $i$-th phase of our algorithm in detail. 
%It has two parts. 

%\paragraph{Part One}
Let $\tG_i$ be the subgraph of $G_i^{< k}$ induced by edges of length exactly $w_i$. 
We apply \cref{thm:large_clustering} on the cluster graph $\pi^{-1}(\tG_i)$. 
This extends the clustering $F_i^{<k}$ to a new clustering $\tF_i$. 
Let $\tF_i^{\ge k}$ contain all connected components $T$ of $\tF_i$ such that their size is at least $k$, that is, $|\pi_i^{-1}(T)| \ge k$. Set $\tF_i^{< k} = \tF_i \setminus \tF_i^{\ge k}$.  

We now define $F_{i+1}$. 
It contains three types of edges:
\begin{enumerate}
    \item First, it contains all edges of $F_i$.
    \item Second, for every edge $e' \in \tF_i$, we take any edge $e \in \pi_i^{-1}(e')$ with $w(e) = w(e')$ and add it to $F_{i+1}$. 
    \item Third, for every connected component $T \subseteq \tF_i^{< k}$, if there is at least one edge $e'$ of weight $w_i$ connecting it with a node from $G_i^{\ge k} \cup \tF_i^{\ge k}$, \todo{careful here, we do not use the right term} we take arbitrary $e \in \pi_i^{-1}(e')$ with $w(e) = w(e')$ and add $e$ to $F_{i+1}$. 

\end{enumerate}
Note that the definition of $F_{i+1}$ also defines the contracted graph $G_{i+1}$ for the next phase of the algorithm. 

%\paragraph{Part Two}
%Consider the graph $G_i^{rem} = G_i[V(G_i) \setminus \tF_i^{\ge k}] / \tF_i^{< k}$. %Note that $G_i^{rem}$ does not contain any edge of weight $w_i$. 

%For any connected component $C'$ of $G_i^{rem}$ of node-weighted size at most $k$, we find a minimum spanning forest $T$ of it and the shortest edge $e$ connecting $C'$ with some $u \in G_i[\tF_i^{\ge k}]$. Such an edge needs to exists due to invariant (2). 
%For all such components $C'$, we add $T$ and $e$ to $\tF_i$, which defines a new forest $\tF_i'$. 

%We set $F_{i+1} = F_i \cup \tF_i'$ and $G_{i+1} = G_i[V(G_i) \setminus V(\tF_{i+1}^{\ge k})] / (\tF_{i+1}^{< k})$. That is, we remove large components of $\tF_i$ from $G_i$ and contract the small components of $\tF_i$. 

This finishes the description of the $i$-th phase of the algorithm and, hence, the whole algorithm. 

\begin{claim}
\label{cl:sanity}
$F_i$ is a forest and contains only edge of weight smaller than $w_i$. 
\end{claim}
\begin{proof}
Follows from construction. 
\end{proof}

We can think of each $T \in F_{i+1}^{\ge k}$ as follows: $\pi_i(T)$ consists of $T_0 \subseteq  F_i \cup \tF_{i}^{\ge k}$ such that $|T_0| \ge k$. 
Next, $T \setminus T_0$ splits into several connected components. Each such component consists of a tree $T_j, j \ge 1$ with $|T_j| < k$ and $T_j$ is connected to $T_0$ via an edge $e_j$ of weight $w_i$, where $e_j$ is the edge of the third type in the definition of $F_{i+1}$. 


\begin{claim}
\label{cl:ruling}
Invariant 3 is satisfied. That is, every connected component $T$ in $F_i$ has diameter at most $O(k \log n) + i \cdot O(k)$ in $G$. 
\end{claim}
\begin{proof}
We prove this by induction. It holds for $i = 0$. Assume it holds for $i$ and consider any $T \subseteq F_{i+1}$.
If $T \subseteq F_i$, we are done by induction and if $T \subseteq F_{i+1}^{< k}$ we have $\hopdiam(T) \le |T| \le k$ by definition, so assume that $T$ contains at least one edge $e \in F_{i+1} \setminus F_i$ and $T \subseteq F_{i+1}^{\ge k}$. 

By discussion above the claim, we can think of $T$ as the core tree $T_0$ connected to additional trees $T_j$, $j \ge 1$. 

Note that either $T_0 \subseteq F_i$ and by induction 
\[
\hopdiam(T_0) \le O(k \log n) + i \cdot O(k),
\]
or $\pi(T_0) \subseteq \tF_i^{\ge k}$ and $\hopdiam(T_0) \le k \cdot \hopdiam(\pi_i(T_0))$ as each node $u \in V(\pi_i(T_0))$ has $|\pi^{-1}_i(u)| < k$. Since $S_i$ is $k \cdot O(\log n)$-ruling, we get 
\[
\hopdiam(T_0) \le k \cdot k \cdot O(\log n) \le O(k \log n). 
\]

For each $T_j, j \ge 1$ we have $\pi_i(T_j) \subseteq \tF_i^{< k}$, hence $\hopdiam(T_j) < k$. This means
\begin{align*}
\hopdiam(T) 
&\le \hopdiam(T_0) + 2(1 + \max_{j \ge 1} \hopdiam(T_j))\\
&\le     O(k \log n) + i \cdot O(k) + O(k)\\
&=      O(k \log n) + (i+1) \cdot O(k) 
\end{align*}
as needed. 

\begin{comment}
There are two possibilities. 
Either we have $\pi_i(T) \subseteq \tF_i^{< k}$, hence $\hopdiam(T) \le |T| < k$. 
Or we have $\pi_i(T) \subseteq$
\begin{enumerate}
\item 
\item $e \in E(\tF_i^{\ge k})$. In this case, $\pi_i(T) \subseteq \tF_i^{\ge k}$ and by \cref{lem:ruling_set} we get that the hop diameter of $\pi_i(T)$ in $G_i$ is bounded by $O(k \log n)$. As each node $u \in V(T_i)$ satisfies $|\pi^{-1}(u)| < k$, we have $\hopdiam(T) \le k \cdot O(k \log n) = O(k^2 \log n)$, as needed.  
\item $e$ connects some $T_1 \subseteq T, \pi_i(T_1) \subseteq F_i^{\ge k}$ with some $T_2$ with $\pi_i(T_2) \subseteq \tF_i^{< k}$. 
    In this case, we know by induction that $\hopdiam(T_1) \le O(k^2 \log n) + i \cdot O(k)$. Besides $T_2$, there can be several new trees $T'$ with $\pi_F(T')$ joined with $T_1$, however, each such tree $T'$ satisfies $\pi_i(T') \subseteq \tF_i^{< k}$, hence $\hopdiam(T_2) \le |T_2| \le k$ and $\hopdiam(T) \le O(k^2 \log n) + (i+1) \cdot O(k)$. 
\end{enumerate}
\end{comment}
%First, suppose that $T \in \tF_i$. 
%It can be split as $C = T_0 \cup \bigcup_{i \ge 1} T_i$ where $T_0$ is the original connected component of $\tF_i^{\ge k}$ and $T_1, T_2, \dots$ are subtrees of $T_0$ that are spanning trees of small components in $G_i^{rem}$. 

%Note that the diameter of $T_0$ in $\tG_i$ is $O(k \log n)$ via \cref{lem:ruling_set}. 
%Since each $T_i, i \ge 1$ contains only at most $k$ nodes, we have that the diameter of $T$ in $\tG_i$ is $O(k \log n) + O(k) = O(k \log n)$. 

%Finally, as we have $G_i = G[V(G) \setminus F_i^{\ge k}] / F_i^{<k}$, each node of $G_i$ corresponds to a connected component of $F_i$ of at most $k$ nodes. Hence, the diameter of $C$ in $G$ is at most $O(k \log n) \cdot k = O(k^2 \log n)$, as needed. 
\end{proof}

\begin{claim}
\label{cl:inv1}
Invariant 1 is satisfied. 
\end{claim}
\begin{proof}
We prove this by induction. 
Consider any edge $e = \{u, v\} \in E(G_i)$ with weight $w_i$. We prove that whenever $e \in E(G_{i+1})$, then $e \in E(G_{i+1}^{\ge k})$. 
We consider several possibilities. 

If $e \in \tF_i$, then by definition $e \not\in E(G_{i+1})$. 
Otherwise, $e$ connects two different connected components $T_1, T_2$ of $F_i \cup \tF_i$. If $T_1, T_2 \subseteq F_{i+1}^{\ge k}$, we are done as $e \in E(G_{i+1}^{\ge k})$. 
Otherwise, at least one of the two connected components, say $T_1$, has size less than $k$. 
If $T_2$ has size at least $k$, then we add at least one edge $f$ connecting $T_1$ to some $T' \subseteq F_{i}^{\ge k}$. Hence, $e$ connects two components of size at least $k$ in $F_{i+1}$. 
Finally, if $|T_2| < k$, then take some $s_1 = T_1 \cap S_i$ and $s_2 = T_2 \cap S_i$. 
We have $d_{G_i}(s_1, s_2) \le |T_1| + 1 + |T_2| \le  3k$. 
This is, however, a contradiction with the fact that $S$ is a $(3k, O(\log n)\cdot k)$-ruling set. 
\end{proof}

\begin{claim}
\label{cl:inv2}
Invariant 2 is satisfied. 
\end{claim}
\begin{proof}
We prove it by induction. At the beginning $F_0$ is an empty forest that trivially satisfies the pretty property. Suppose the claim holds for $i$ and we prove it for $i+1$. 

Take any connected component $T \subseteq F_{i+1}$. We consider two cases. 
First suppose that $T \subseteq F_{i+1}^{< k}$. Take any $u, v \in V(T)$. If $\pi_{i-1}(u) = \pi_{i-1}(v)$, then $u,v$ belong to the same connected component of $F_i$ and we use induction. 
Otherwise, we choose $C_{uv} = \pi_{i-1}^{-1}(\pi_{i-1}(u))$. That is, $C_{uv}$ is the tree that contracted to the node $\pi_{i-1}(u)$ in $G_i$. Our assumption $\pi_{i-1}(u) \not= \pi_{i-1}(v)$ implies $v \not\in C_{uv}$. Note that the shortest path $P \subseteq T$ connecting $u$ and $v$ has all weights at most equal to $w_i$ via \cref{cl:sanity}. 
That is, 
\[
\max_{e \in P} w(e) \le w_i
\]
On the other hand, Invariant 1 implies that there any edge in $G_i$ incident to $\pi_F(u)$ has weight at least $w_i$ -- otherwise, we would get that $u \in G_i^{\ge k}$ contradicting the fact that $T \subseteq F_{i+1}^{< k}$. Hence, 
\[
\min_{e \in C_{uv} \times (V(G) \setminus C_{uv})} w(e) \ge w_i
\]
We are getting
\[
\max_{e \in P} w(e) \le \min_{e \in C_{uv} \times (V(G) \setminus C_{uv})} w(e)
\]
which finishes the proof for $T \subseteq F_{i+1}^{< k}$. 

Next, assume $T \subseteq F_{i+1}^{\ge k}$. Recall that we can think of $T$ as containing a center tree $T_0$ and appended trees $T_j, j \ge 1$. We again consider several cases. If $\pi_{i-1}(u) = \pi_{i-1}(v)$, we use induction. 
Otherwise, for the path $P$ connecting $u$ and $v$ in $T$ we have
\[
\max_{e \in P} w(e) \le w_i
\]
by \cref{cl:sanity}. 
We next consider three cases. 
\begin{enumerate}
    \item If $u, v \in T_0$, then by our assumption $\pi_{i-1}(u) \not= \pi_{i-1}(v)$ we get $T_0 \not\subseteq F_{i-1}^{\ge k}$, hence by Invariant 1, there is no edge leaving $T_0$ of weight less than $w_i$. Hence, taking $C_{uv} = \pi^{-1}_{i-1}(\pi_{i-1}(u))$ satisfies $v \not\in C_{uv}$ and 
\[
\min_{e \in C_{uv} \times (V(G) \setminus C_{uv})} w(e) \ge w_i
\]
    \item If $u, v \in T_j$ for $j \ge 1$, we argue the same as in previous bullet point, the fact $|T_j| < k$ and Invariant 1 imply there is no edge of weight smaller than $w_i$ leaving $\pi_{i-1}^{-1}(\pi_{i-1}(u))$. 
    \item 
If at least one of $u,v$, say $u$, is in $T_j$ for $j \ge 1$ and $v \not\in T_j$, consider $C_{uv} = V(T_j)$. We have $v \not\in C_{uv}$ and since $|T_j|<k$, we can apply Invariant 1 and again get 
\[
\min_{e \in C_{uv} \times (V(G) \setminus C_{uv})} w(e) \ge w_i
\]
\end{enumerate}
In all cases, we get 
\[
\max_{e \in P} w(e) \le \min_{e \in C_{uv} \times (V(G) \setminus C_{uv})} w(e)
\]
as needed. 
\end{proof}

\begin{claim}
\label{cl:small}
$F_b = F_b^{\ge k}$. 
\end{claim}
\begin{proof}
Suppose the contrary, i.e., $F_b^{< k}$ is nonempty and let $u \in F_b^{<k}/F_b^{<k} \subseteq G_b$. 
By invariant 1, this implies that there are no edges from $u$ to other nodes in $G_b$. Since $|\pi_b^{-1}(u)|<k$, this implies that $G$ contains a connected component of size smaller than $k$, a contradiction with our assumption that $G$ is connected and $n \ge k$. 
\end{proof}


\begin{claim}
\label{cl:time}
The algorithm finishes in $\poly(k \log n)$ \congest rounds. 
\end{claim}
\begin{proof}
\end{proof}

By \cref{cl:small,cl:inv2} the output of our algorithm has the desireable properties. 
By \cref{cl:time}, the algorithm finishes in $\poly(k \log n)$ \congest rounds, as needed. 

\end{proof}
\end{comment}

























\begin{restatable}{theorem}{weighted}
\label{thm:weighted_spanner}
Suppose that there are functions $\aus(n,k), \Tus(n,k)$ such that for every $n,k$ there exists a deterministic (randomized) algorithm that constructs an $\aus(n,k)$-spanner of an unweighted graph with at most $n + n/k$ edges in $\Tus(n,k)$ \congest rounds. 

Then there is a deterministic (randomized) \congest algorithm that, given an input weighted graph $G$ with edge-weights from $[n^{O(1)}]$ and a parameter $k$, constructs a weighted $\beta$-spanner $H$ of $G$ with
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
    \item $|E(H)| \le n + O(\frac{n\log n}{k})$,
    \item $\beta = O(\aus(n,k) \cdot \log^2 n)$.
\end{enumerate}
in $\Tus(n,k) \cdot O(\log^? n)$ \congest rounds. 
\end{restatable}

